ProAV-DiT: A Projected Latent Diffusion Transformer for Efficient Synchronized Audio-Video Generation

Sounding Video Generation (SVG) remains a challenging task due to the inherent structural misalignment between audio and video, as well as the high computational cost of multimodal data processing. In this paper, we introduce ProAV-DiT, a Projected Latent Diffusion Transformer designed for efficient and synchronized audio-video generation. To address structural inconsistencies, we preprocess raw audio into video-like representations, aligning both the temporal and spatial dimensions between audio and video. At its core, ProAV-DiT adopts a Multi-scale Dual-stream Spatio-Temporal Autoencoder (MDSA), which projects both modalities into a unified latent space using orthogonal decomposition, enabling fine-grained spatiotemporal modeling and semantic alignment. To further enhance temporal coherence and modality-specific fusion, we introduce a multi-scale attention mechanism, which consists of multi-scale temporal self-attention and group cross-modal attention. Furthermore, we stack the 2D latents from MDSA into a unified 3D latent space, which is processed by a spatio-temporal diffusion Transformer. This design efficiently models spatiotemporal dependencies, enabling the generation of high-fidelity synchronized audio-video content while reducing computational overhead. Extensive experiments conducted on standard benchmarks demonstrate that ProAV-DiT outperforms existing methods in both generation quality and computational efficiency.

==> fig/fig1.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Fig/fig1.pdf}
    \caption{Existing Audio-Video Generation methods.}
    \vspace{-15pt}
    \label{exist-svg-method}
\end{figure}


==> fig/fig6.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Fig/fig4.pdf}
    \caption{Results of our method on Landscape, including spectrogram visualization images and video frames.}
    \label{landscape-results}
    \vspace{-3ex}
\end{figure*} 


==> table/tab5.tex <==
\begin{table}[h] % [h] 尝试将表格放在此处
    \centering
    \caption{Ablation study of MDSA (ProAV-DiT) on the Landscape dataset}
    \scalebox{0.85}{
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} &
        \textbf{rFVD}$\downarrow$ & % 添加下降箭头表示越低越好
        \textbf{rKVD}$\downarrow$ &
        \textbf{FAD}$\downarrow$ \\
        \midrule
        % PVDM & 70.2 & 4.1 & 9.0 \\
        % MM-LDM & 53.9 & 2.4 & 8.9 \\
        % \midrule
        \textbf{MDSA (ProAV-DiT)} & \textbf{29.5} & \textbf{1.3} & \textbf{8.5} \\
        \multicolumn{4}{c}{\cellcolor{gray!15} Multi-scale attention mechanism ablation}\\
        $-$ MT-selfAttn & 35.1 & 2.2 & 8.6 \\
        $-$ GCM-Attn & 39.2 & 2.3 & 8.7 \\
        $-$ Bi-Block CrossAttn & 45.6 & 2.4 & 8.8 \\
        \multicolumn{4}{c}{\cellcolor{gray!15} Other ablations (Losses)} \\
        $-$ finetune with KL loss & 60.2 & 3.2 & 8.9 \\
        $-$ adversarial loss & 134.5 & 8.3 & 9.8 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:ablation-pavdit}
    \vspace{-2ex}
\end{table}

==> table/tab7.tex <==
\begin{table}[h] % [h] 尝试将表格放在此处
    \centering
    \caption{Ablation study of MDSA (PAV-DiT) on the Landscape dataset}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} &
        \textbf{rFVD}$\downarrow$ & % 添加下降箭头表示越低越好
        \textbf{rKVD}$\downarrow$ &
        \textbf{FAD}$\downarrow$ \\
        \midrule
        PVDM & 70.2 & 4.1 & 9.0 \\
        MM-LDM & 53.9 & 2.4 & 8.9 \\
        \midrule
        \textbf{MDSA (PAV-DiT)} & \textbf{29.5} & \textbf{1.3} & \textbf{8.5} \\
        \multicolumn{4}{@{}l}{\cellcolor{gray!15}multi-scale attention mechanism ablation}\\
        $-$ MT-selfAttn & 35.1 & 2.2 & 8.6 \\
        $-$ GCM-Attn & 39.2 & 2.3 & 8.7 \\
        $-$ Bi-Block CrossAttn & 45.6 & 2.4 & 8.8 \\
        \multicolumn{4}{@{}l}{\cellcolor{gray!15} Other ablations (Losses)} \\
        $-$ finetune with KL loss & 60.2 & 3.2 & 8.9 \\
        $-$ adversarial loss & 134.5 & 8.3 & 9.8 \\
        \bottomrule
    \end{tabular}
    \label{tab:ablation-pavdit}
\end{table}

==> table/tab8.tex <==
\begin{table}[t]
\centering
% \vspace{-3ex} % 保持排版简洁，去除不必要的硬编码垂直间距
\caption{Comparison of Reconstruction on the AIST++ Dataset.} % 优化标题以更清晰地说明是重建性能
\label{tab:pvdm-comparion}
\scalebox{0.85}{
\begin{tabular}{lcccc} 
\toprule
\textbf{Method} & \textbf{FVD}$\downarrow$ & \textbf{FAD}$\downarrow$ & \textbf{PSNR-A}$\uparrow$ & \textbf{PSNR-V}$\uparrow$ \\ % 统一指标方向
\midrule
MM-LDM  & 53.9 & 8.9 & - & -  \\
\midrule
% Ablation for clarity (Optional, based on original content)
MDSA-V  & 30.3 & - & - & 31.34 \\ % 仅视频重建（可能用于消融对比）
MDSA-A  & - & 9.4 & 35.93 & - \\ % 仅音频重建（可能用于消融对比）
\tableLineBlue \textbf{MDSA} & \textbf{18.7} & \textbf{8.7} & \textbf{37.33} & \textbf{32.19} \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/table.tex <==



\begin{table*}[t]
\centering
% \small 
\caption{Quantitative performance comparison of multimodal video generation models on Landscape and AIST++ datasets. Results with $*$ are reproduced using released sources.}
\scalebox{0.8}{
% \begin{tabular}{l|c|c|ccc|ccc}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Resolution}} & \multirow{2}{*}{\textbf{Sampler}} & \multicolumn{3}{c|}{\textbf{Landscape}} & \multicolumn{3}{c}{\textbf{AIST++}} \\
% & & & FVD $\downarrow$ & KVD $\downarrow$ & FAD $\downarrow$ & FVD $\downarrow$ & KVD $\downarrow$ & FAD $\downarrow$ \\
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Resolution}} & \multirow{2}{*}{\textbf{Sampler}} & \multicolumn{3}{c}{\textbf{Landscape}} & \multicolumn{3}{c}{\textbf{AIST++}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9} % 添加分组横线
& & & FVD $\downarrow$ & KVD $\downarrow$ & FAD $\downarrow$ & FVD $\downarrow$ & KVD $\downarrow$ & FAD $\downarrow$ \\
% \midrule
\midrule
% \multicolumn{9}{c}{\textbf{Single-Modal Video Generation}} \\
% \midrule
\multicolumn{9}{@{}c@{}}{\cellcolor{gray!30} Single-Modal Video Generation} \\ 
% \addlinespace[-2pt] 
% \midrule[0.5pt] 
\hdashline
DIGAN*              & 64$^2$ & -                 & 305.4 & 19.6  & -   & 119.5 & 35.8  & - \\
TATS-base*           & 64$^2$ & -                 & 600.3 & 51.5  & -   & 267.2 & 41.6  & - \\
MM-Diffusion-v*                  & 64$^2$ & dpm-solver        & 237.9 & 13.9  & -   & 163.1 & 28.9  & - \\
MM-Diffusion-v+SR*               & 64$^2$ & dpm-solver+DDIM   & 225.4 & 13.3  & -   & 142.9 & 24.9  & - \\
MM-LDM-v*                         & 64$^2$ & DDIM              & 122.1 & 6.4   & -   & 83.1  & 13.1  & - \\
MM-Diffusion-v+SR*               & 256$^2$ & dpm-solver+DDIM  & 347.9 & 27.8  & -   & 225.1 & 51.9  & - \\
MM-LDM-v*                         & 256$^2$ & DDIM             & 156.1 & 13.0  & -   & 120.9 & 26.5  & - \\
PAV-DiT-v                        & 256$^2$ & Reflect Flow     & \textbf{90.9}  & \textbf{7.8} & -   & \textbf{84.2} & \textbf{13.3} & - \\
\midrule
\multicolumn{9}{@{}c@{}}{Multi-Modal Generation} \\ % 同样修复
% \addlinespace[-2pt]
% \midrule[0.5pt]
\hdashline
% \midrule
MM-Diffusion-svg+SR*            & 64$^2$ & dpm-solver+DDIM  & 211.2 & 12.6  & 9.9  & 137.4 & 24.2  & 12.3 \\
% MM-LDM-a2v*                       & 64$^2$ & DDIM             & 89.2  & 4.2   & -    & 71.0  & 10.8  & - \\
% MM-LDM-v2a*                       & -      & DDIM             & -     & -     & 9.2  & -     & -     & 10.2 \\
MM-LDM-svg*                       & 64$^2$ & DDIM             & 77.4 & 3.2 & 9.1 & 55.9 & 8.2 & 10.2 \\
% \midrule
\hdashline
MM-Diffusion-svg+SR*            & 256$^2$ & dpm-solver+DDIM  & 332.1 & 26.6  & 9.9  & 219.6 & 49.1  & 12.3 \\
% MM-LDM-a2v*                       & 256$^2$ & DDIM             & 123.1 & 10.4  & -    & 128.5 & 33.2  & - \\
MM-LDM-svg*                       & 256$^2$ & DDIM             & 105.0 & 8.3   & 9.1  & 105.0 & 27.9  & 10.2 \\
AV-DiT*                           & 256$^2$  & -                & 172.7 & 15.4  & 11.2 & 68.8  & 21.0  & 10.2 \\
% \midrule
\hdashline
PAV-DiT wo/text         & 256$^2$ & Reflect Flow     & 87.3  & 7.7   & 8.7  & 85.6  & 19.8  & 9.8 \\
PAV-DiT                 & 256$^2$ & Reflect Flow     & \textbf{80.3}  & \textbf{7.3} & \textbf{8.5}  & \textbf{77.6} & \textbf{18.2} & \textbf{9.4} \\
\midrule
\multicolumn{9}{@{}c@{}}{200 Samples (Follow the See\&Hear experimental setup)} \\ % 同样修复
% \addlinespace[-2pt]
% \midrule[0.5pt]
\hdashline
See\&Hear*                        & 256$^2$ & -                & 326.2 & 9.2   & 12.7 & -     & -     & - \\
AV-DiT*                        & 256$^2$ & -                & 260.5 & 9.2 & 14.1 & -     & -     & - \\
\tableLineColor PAV-DiT                          & 256$^2$ & Reflect Flow     & \textbf{240.3} & \textbf{9.0} & \textbf{12.2} & -     & -     & - \\
\bottomrule
\end{tabular}
}
\vspace{-4ex}
\label{tab:comparison}
\end{table*}





\begin{table}[t]
    \centering
        \centering
        \caption{Quantitative comparison with scaled-up data and model for open-domain generation.}
        \vspace{-1ex}
        \label{tab:scale}
        \scalebox{0.85}{
        \begin{tabular}{l c c c c}
        \toprule
        \textbf{Model} & \textbf{\#P} & 
        \multicolumn{1}{c}{\textbf{FVD}$\downarrow$} & 
        \multicolumn{1}{c}{\textbf{KVD}$\downarrow$} & 
        \multicolumn{1}{c}{\textbf{FAD}$\downarrow$} \\
        \midrule
        MM-Diffusion   & 134M    & 649.8 & 34.6 & 2.9 \\
        MM-LDM-S       & 131M    & 185.8 & 10.1 & 1.59 \\
        MM-LDM-B       & 384M    & 181.5 & 9.5  & 1.55 \\
        MM-LDM-L       & 1543M   & 164.1 & 8.5  & 1.52 \\
        PAV-DiT        & 702M    & 148.7 & 8.4  & 1.51 \\
        \bottomrule
        \end{tabular}
        }
\end{table}







\begin{table}[t]
        \centering
        \caption{Efficiency comparison of PAV-DiT with MM-Diffusion and MM-LDM.}
         \vspace{-1ex}
        \label{tab:efficiency}
        \scalebox{0.8}{
        \begin{tabular}{@{}l c >{\centering\arraybackslash}p{1.8cm} >{\centering\arraybackslash}p{1.8cm}@{}}
        \toprule
        \textbf{Method} & \textbf{Res.} & \textbf{Train/Step} & \textbf{Infer/Sample} \\
        \midrule
        MM-Diffusion          & $64^2$    & 1.70s  & 33.8s \\
        MM-Diffusion          & $128^2$   & 2.36s  & 90.0s \\
        % \midrule
        MM-LDM         & $256^2$   & 0.46s  & 70.0s \\
        MM-LDM*        & $256^2$   & 0.38s  & 8.7s  \\
        % \midrule
        PAV-DiT (ours)        & $256^2$   & 0.44s  & 17.7s \\
        PAV-DiT* (ours)       & $256^2$   & \textbf{0.32s}  & \textbf{3.93s} \\
        \bottomrule
        \end{tabular}
        }
    \vspace{-3ex}
\end{table}



\begin{wraptable}{r}{0.45\textwidth}
    \vspace{-3ex}
    \centering
    \small % 使用较小字体
    \caption{Human Evaluation Results}
    \begin{tabular}{lccc}
    \toprule
    \textbf{Method} & \textbf{AQ}$\uparrow$ & \textbf{VQ}$\uparrow$ & \textbf{A-V}$\uparrow$ \\
    \midrule
    MM-Diffusion    & 2.46  & 2.10    & 2.99      \\
    MM-LDM          & 2.98  & 3.68    & 3.29      \\
    \midrule
    PAV-DiT         & 3.22  & 3.97    & 3.60      \\
    \bottomrule
    \end{tabular}
    \label{human}
    % \vspace{-8pt}
\end{wraptable}



\begin{wraptable}{r}{0.45\textwidth}    
\vspace{-3ex}
    \centering
    \caption{Ablation study of MDSA (PAV-DiT) on the Landscape dataset} 
    \scalebox{0.85}{
        \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Model} & 
        \multicolumn{1}{c}{\textbf{rFVD}} & 
        \multicolumn{1}{c}{\textbf{rKVD}} & 
        \multicolumn{1}{c}{\textbf{FAD}} \\
        \midrule
        PVDM & 70.2 & 4.1 & 9.0 \\
        MM-LDM & 53.9 & 2.4 & 8.9 \\
        \midrule
        \textbf{MDSA (PAV-DiT)} & \textbf{29.5} & \textbf{1.3} & \textbf{8.5} \\
        \multicolumn{4}{@{}l}{\textit{multi-scale attention mechanism}} \\
        $-$ MT-selfAttn & 35.1 & 2.2 & 8.6 \\
        $-$ GCM-Attn & 39.2 & 2.3 & 8.7 \\
        $-$ Bi-Block CrossAttn & 45.6 & 2.4 & 8.8 \\
        \multicolumn{4}{@{}l}{\textit{Other ablations:}} \\
        $-$ finetune with KL loss & 60.2 & 3.2 & 8.9 \\
        $-$ adversarial loss & 134.5 & 8.3 & 9.8 \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:ablation-pavdit}
    \vspace{-8pt}
\end{wraptable}
